A New Approach to the Small Phylogeny Problem

In the small phylogeny problem we, are given a phylogenetic tree and gene orders of the extant species and our goal is to reconstruct all of the ancestral genomes so that the number of evolutionary operations is minimized. Algorithms for reconstructing evolutionary history from gene orders are usually based on repeatedly computing medians of genomes at neighbouring vertices of the tree. We propose a new, more general approach, based on an iterative local optimization procedure. In each step, we propose candidates for ancestral genomes and choose the best ones by dynamic programming. We have implemented our method and used it to reconstruct evolutionary history of 16 yeast mtDNAs and 13 Campanulaceae cpDNAs.

==> Makefile <==
all: main.pdf

clean:
	-rm main.aux main.bbl main.blg main.log main.log main.lot main.out \
	main.dvi main.ps main.pdf *~

main.ps: main.dvi
	dvips main -o main.ps

main.pdf: main.tex *.tex *.bib
	pdflatex main
	pdflatex main
	-bibtex main
	pdflatex main
	pdflatex main

main.dvi: main.tex *.tex *.bib
	latex main
	latex main
	-bibtex main
	latex main
	latex main

.PHONY: all bib

